Taming Complexity in Intuitionistic Modal Logic: The Case of FIK and Its Shallow Calculus

Intuitionistic modal logics (IMLs) comprise many systems: from constructive modal logics such as CK and Wijesekera's CCDL to Fischer Servi/Simpson's IK, as well as some recently introduced variants. All of them are characterized by bi-relational semantics and have complete axiomatisations. However, from the perspective of proof theory and complexity, there are strong differences: while for constructive modal logics simple Gentzen calculi suffice, for IK more complex calculi, based on nested or labelled sequents, are needed. As a consequence, the decision problem for constructive modal logics has a PSPACE upper bound, whereas for IK is not known and it is even conjectured to be non-elementary. We study here the proof theory and complexity of FIK, a natural intuitionistic modal logic recently introduced. FIK is strictly in between CCDL and IK, yet it has the same forcing conditions as IK. We define a "shallow" sequent calculus for FIK which is a nested sequent calculus where sequents have at most one level of nesting. We prove its syntactic completeness by showing the admissibility of cut. By means of this calculus we show that decision problem for FIK is in EXPSPACE, whence significantly lower than the complexity conjectured for IK.

==> eptcsdata.tex <==
\providecommand{\firstpage}{407}
\providecommand{\publicationstatus}{M.~B\'ilkov\'a, M.~Gattinger, I.~van~der~Giessen, M.~Girlando, Y.~Wang (Eds.):\\
Advances in Modal Logic 2026 (AiML 2026)\\
EPTCS 447, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.447.23}{10.4204/EPTCS.447.23}}

